On conducting better validation studies of automatic metrics in natural language generation evaluation

Natural language generation (NLG) has received increasing attention, which has highlighted evaluation as a central methodological concern. Since human evaluations for these systems are costly, automatic metrics have broad appeal in NLG. Research in language generation often finds situations where it is appropriate to apply existing metrics or propose new ones. The application of these metrics are entirely dependent on validation studies - studies that determine a metric's correlation to human judgment. However, there are many details and considerations in conducting strong validation studies. This document is intended for those validating existing metrics or proposing new ones in the broad context of NLG: we 1) begin with a write-up of best practices in validation studies, 2) outline how to adopt these practices, 3) conduct analyses in the WMT'17 metrics shared task\footnote{Our jupyter notebook containing the analyses is available at \url{https://github.com}}, and 4) highlight promising approaches to NLG metrics 5) conclude with our opinions on the future of this area.

==> notes.tex <==
\begin{comment}
\begin{enumerate}
    % read the video captioning DA paper?
    \item After WMT'16, the human evaluation campaign for the translation shared task adopts Direct Assessment. \cite[DA;][]{DBLP:conf/naacl/GrahamBM15} DA is a score averaged over $n$ human judgments on a 1-6 Likert scale to consistently estimate the population mean of each translation's quality, where $n$ is determined empirically. In MT, $n=15$ has been found to be sufficient. More on DA in \S 3.2. A ranking of systems is produced by averaging the segment-level DA scores for each system. More on system-level rankings in \S 2.1.
    
    \item Participating researchers develop their metric submission with previous years' data for training/validation as needed. Note that the annotation scheme varies over years.
    
    \item System translations and references are tokenized and released as a test set. Researchers produce scores from metrics for evaluation.
    
    \item System and segment-level results are computed in the form of Pearson correlations. More on the use of Pearson correlation in \S 2.2. With Pearson correlation, a William's test \cite{williams1959regression,DBLP:conf/emnlp/GrahamB14} can be conducted to measure whether an increase in correlation of a metric with human judgment is significant or by chance. This test tests whether $Corr(X_1, X_3) = Corr(X_2, X_3)$, where $X_1$ and $X_2$ are correlated. In our case, $X_1$ and $X_2$ are generalizations of two different metric scores, and $X_3$ of translation DA scores.
\end{enumerate}

\item Use scalar scoring judgments. Reasons to use scalar judgments over ranking judgments are partially outlined in \S 2.2. \citet{DBLP:conf/naacl/GrahamBM15} found that averages over a sufficient number of scalar human judgments are found to be consistent and replicable.
    
    \item Determine the sufficient number of judgments per segment empirically as in \citet{DBLP:conf/naacl/GrahamBM15}. This involves running a pilot study on a subset of your dataset where a large number (i.e. $n=100$) of judgments are collected per segment. Compute average DA scores for each segment with the first $i$ judgments, and estimate a true mean with the remaining $n-i$ judgments. For the $i$ where the correlation between DA scores and ``true mean'' is sufficient, gather $i$ judgments for each segment in the full data collection.
\end{comment}
